Automatic Evaluation of Healthcare LLMs Beyond Question-Answering

Current Large Language Models (LLMs) benchmarks are often based on open-ended or close-ended QA evaluations, avoiding the requirement of human labor. Close-ended measurements evaluate the factuality of responses but lack expressiveness. Open-ended capture the model's capacity to produce discourse responses but are harder to assess for correctness. These two approaches are commonly used, either independently or together, though their relationship remains poorly understood. This work is focused on the healthcare domain, where both factuality and discourse matter greatly. It introduces a comprehensive, multi-axis suite for healthcare LLM evaluation, exploring correlations between open and close benchmarks and metrics. Findings include blind spots and overlaps in current methodologies. As an updated sanity check, we release a new medical benchmark --CareQA-- with both open and closed variants. Finally, we propose a novel metric for open-ended evaluations -- Relaxed Perplexity -- to mitigate the identified limitations.

==> latex/tables/close_ended_old.tex <==
\begin{table*}[h]
\centering
\renewcommand{\arraystretch}{1.5} 
\resizebox{2.1\columnwidth}{!}{%
\begin{tabular}{l|ccccccccc}
\toprule
\textbf{Model} & \multicolumn{9}{c}{\textbf{Close-ended}} \\ 
 & \textbf{MedMCQA $\uparrow$} & \textbf{MedQA $\uparrow$} & \textbf{\careqa{} $\uparrow$} & \textbf{multimedqa $\uparrow$} & \textbf{PubMedQA $\uparrow$} & \textbf{Med Text Classification $\uparrow$} & \textbf{Med Transcriptions $\uparrow$} & \textbf{BioRED $\uparrow$} & \textbf{MMLU $\uparrow$} \\ 
\midrule
BioMistral-MedMNX & 0.495 ± 0.008 & 0.515 ± 0.014 & 0.629 ± 0.006 & 0.547 ± 0.006 & 0.776 ± 0.019 & 0.202 ± 0.011 & 0.356 ± 0.007 & 0.216 ± 0.013 & 0.6784 ± 0.034 \\
JSL-MedLlama-3-8B-v2.0 & 0.613 ± 0.008 & 0.617 ± 0.014 & 0.671 ± 0.006 & 0.648 ± 0.006 & 0.742 ± 0.020 & 0.191 ± 0.010 & 0.361 ± 0.007 & 0.254 ± 0.014 & 0.7739 ± 0.0305 \\
Llama3-Med42-8B & 0.603 ± 0.008 & 0.626 ± 0.014 & 0.684 ± 0.006 & 0.642 ± 0.006 & 0.772 ± 0.019 & 0.202 ± 0.011 & 0.377 ± 0.007 & 0.203 ± 0.013 & 0.7525 ± 0.0315 \\
Meta-Llama-3.1-70B-Instruct & 0.722 ± 0.007 & 0.798 ± 0.011 & 0.836 ± 0.005 & 0.764 ± 0.005 & 0.800 ± 0.018 & 0.145 ± 0.003 & 0.381 ± 0.007 & 0.515 ± 0.016 & 0.8711 ± 0.0236 \\
Meta-Llama-3.1-8B-Instruct & 0.593 ± 0.008 & 0.637 ± 0.013 & 0.703 ± 0.006 & 0.638 ± 0.006 & 0.752 ± 0.019 & 0.161 ± 0.003 & 0.334 ± 0.007  & 0.232 ± 0.013 & 0.7621 ± 0.031 \\
Mistral-7B-Instruct-v0.3 & 0.482 ± 0.008 & 0.523 ± 0.014 & 0.607 ± 0.007 & 0.538 ± 0.006 & 0.774 ± 0.019 & 0.178 ± 0.010 & 0.356 ± 0.007 & 0.358 ± 0.015 & 0.661 ± 0.0345 \\
Mixtral-8x7B-Instruct-v0.1 & 0.564  ± 0.008	&  0.614  ± 0.014 & 0.725 ± 0.006   & 0.622  ± 0.006 & 0.796  ± 0.018 & 0.207  ± 0.011 & 0.344 ± 0.007 & 0.352  ± 0.015 & 0.7766 ± 0.0304  \\
Phi-3-medium-4k-instruct & 0.623 ± 0.007 & 0.596 ± 0.014 & 0.769 ± 0.006 & 0.661 ± 0.006 & 0.782 ± 0.018 & 0.048 ± 0.002 & 0.365 ± 0.007 & 0.261 ± 0.014 & 0.8237 ± 0.0275 \\
Phi-3-mini-4k-instruct & 0.572 ± 0.008 & 0.537 ± 0.014 & 0.700 ± 0.006 & 0.604 ± 0.006 & 0.752 ± 0.019 & 0.192 ± 0.003 & 0.367 ± 0.007 & 0.262 ± 0.014 & 0.7398 ± 0.0321 \\
%Qwen2-72B-Instruct & 0.693 ± 0.007 & 0.768 ± 0.012 & 0.833 ± 0.005 & 0.741 ± 0.005 & 0.794 ± 0.018 & - & - & 0.428 ± 0.016  & - & - & 0.8656 ± 0.0247 \\
Qwen2-7B-Instruct & 0.551 ± 0.008 & 0.570 ± 0.014 & 0.681 ± 0.006 & 0.596 ± 0.006 & 0.742 ± 0.020 & 0.225 ± 0.011 & 0.363 ± 0.007 & 0.197 ± 0.013 & 0.7337 ± 0.032 \\
Yi-1.5-34B-Chat & 0.575 ± 0.008 & 0.614 ± 0.014 & 0.732 ± 0.006 & 0.628 ± 0.006 & 0.774 ± 0.019 & 0.301 ± 0.012 & 0.345 ± 0.007 & 0.543 ± 0.016 & 0.7806 ± 0.0298 \\
Yi-1.5-9B-Chat & 0.488 ± 0.008 & 0.515 ± 0.014 & 0.649 ± 0.006 & 0.546 ± 0.006 & 0.774 ± 0.019 & 0.227 ± 0.011 & 0.330 ± 0.007 & 0.537 ± 0.016 & 0.7007 ± 0.0329 \\
%gemma-2-27b-it & 0.616 ± 0.008 & 0.669 ± 0.013 & 0.781 ± 0.006 & 0.670 ± 0.006 & 0.800 ± 0.018 & 0.222 ± 0.011 & 0.005 ± 0.001 &  0.536 ± 0.016 & 0.220 ± 0.004	& 0.331 ± 0.004 & 0.8163 ± 0.0278 \\
%gemma-2-9b-it & 0.566 ± 0.008 & 0.629 ± 0.014 & 0.745 ± 0.006 & 0.625 ± 0.006 & 0.766 ± 0.019 & 0.209 ± 0.011 & 0.221 ± 0.006 & 0.536 ± 0.016 & 0.230  ± 0.004 & 0.399  ± 0.005 & 0.7796 ± 0.0303 \\
\bottomrule
\end{tabular}
} 
\caption{Close-ended results.}
\label{tab:close_ended_benchmarks}
\end{table*}


\iffalse

\begin{table*}[H]
\centering
\renewcommand{\arraystretch}{1.5} 
\resizebox{2.1\columnwidth}{!}{%
\begin{tabular}{l|ccccccccccc}
\toprule
\textbf{Model} & \multicolumn{11}{c}{\textbf{Close-ended}} \\ 
 & \textbf{MedMCQA $\uparrow$} & \textbf{MedQA $\uparrow$} & \textbf{\careqa{} $\uparrow$} & \textbf{multimedqa $\uparrow$} & \textbf{PubMedQA $\uparrow$} & \textbf{MedText (easy) $\uparrow$} & \textbf{MedText (hard) $\uparrow$} & \textbf{BioRED $\uparrow$} & \textbf{Med Text Classification $\uparrow$} & \textbf{Med Transcriptions $\uparrow$} & \textbf{MMLU $\uparrow$} \\ 
\midrule
BioMistral-MedMNX & 0.495 ± 0.008 & 0.515 ± 0.014 & 0.629 ± 0.006 & 0.547 ± 0.006 & 0.776 ± 0.019 & 0.202 ± 0.011 & 0.356 ± 0.007 & 0.216 ± 0.013 &  0.989 ± 0.001 & 0.942 ± 0.002 & 0.6784 ± 0.034 \\
JSL-MedLlama-3-8B-v2.0 & 0.613 ± 0.008 & 0.617 ± 0.014 & 0.671 ± 0.006 & 0.648 ± 0.006 & 0.742 ± 0.020 & 0.191 ± 0.010 & 0.361 ± 0.007 & 0.254 ± 0.014 & 0.993 ± 0.001 & 0.937 ± 0.002 & 0.7739 ± 0.0305 \\
Llama3-Med42-8B & 0.603 ± 0.008 & 0.626 ± 0.014 & 0.684 ± 0.006 & 0.642 ± 0.006 & 0.772 ± 0.019 & 0.202 ± 0.011 & 0.377 ± 0.007 & 0.203 ± 0.013 &  0.978 ± 0.001 & 0.933 ± 0.002 & 0.7525 ± 0.0315 \\
Meta-Llama-3.1-70B-Instruct & 0.722 ± 0.007 & 0.798 ± 0.011 & 0.836 ± 0.005 & 0.764 ± 0.005 & 0.800 ± 0.018 & 0.145 ± 0.003 & 0.381 ± 0.007 & 0.515 ± 0.016 & 0.987 ± 0.001 & 0.934 ± 0.002 & 0.8711 ± 0.0236 \\
Meta-Llama-3.1-8B-Instruct & 0.593 ± 0.008 & 0.637 ± 0.013 & 0.703 ± 0.006 & 0.638 ± 0.006 & 0.752 ± 0.019 & 0.161 ± 0.003 & 0.334 ± 0.007  & 0.232 ± 0.013 & 0.986 ± 0.001 & 0.929 ± 0.002 & 0.7621 ± 0.031 \\
Mistral-7B-Instruct-v0.3 & 0.482 ± 0.008 & 0.523 ± 0.014 & 0.607 ± 0.007 & 0.538 ± 0.006 & 0.774 ± 0.019 & 0.178 ± 0.010 & 0.356 ± 0.007 & 0.358 ± 0.015 &  0.990 ± 0.001 & 0.941 ± 0.002 & 0.661 ± 0.0345 \\
Mixtral-8x7B-Instruct-v0.1 & 0.564  ± 0.008	&  0.614  ± 0.014 & 0.725 ± 0.006   & 0.622  ± 0.006 & 0.796  ± 0.018 & 0.207  ± 0.011 & 0.344 ± 0.007 & 0.352  ± 0.015 &  0.982  ± 0.001 & 0.937  ± 0.002 & 0.7766 ± 0.0304  \\
Phi-3-medium-4k-instruct & 0.623 ± 0.007 & 0.596 ± 0.014 & 0.769 ± 0.006 & 0.661 ± 0.006 & 0.782 ± 0.018 & 0.048 ± 0.002 & 0.365 ± 0.007 & 0.261 ± 0.014 & 0.990 ± 0.001 & 0.933 ± 0.002 & 0.8237 ± 0.0275 \\
Phi-3-mini-4k-instruct & 0.572 ± 0.008 & 0.537 ± 0.014 & 0.700 ± 0.006 & 0.604 ± 0.006 & 0.752 ± 0.019 & 0.192 ± 0.003 & 0.367 ± 0.007 & 0.262 ± 0.014 & 0.983 ± 0.001 & 0.921 ± 0.003 & 0.7398 ± 0.0321 \\
%Qwen2-72B-Instruct & 0.693 ± 0.007 & 0.768 ± 0.012 & 0.833 ± 0.005 & 0.741 ± 0.005 & 0.794 ± 0.018 & - & - & 0.428 ± 0.016  & - & - & 0.8656 ± 0.0247 \\
Qwen2-7B-Instruct & 0.551 ± 0.008 & 0.570 ± 0.014 & 0.681 ± 0.006 & 0.596 ± 0.006 & 0.742 ± 0.020 & 0.225 ± 0.011 & 0.363 ± 0.007 & 0.197 ± 0.013 &  0.976 ± 0.001 & 0.934 ± 0.002 & 0.7337 ± 0.032 \\
Yi-1.5-34B-Chat & 0.575 ± 0.008 & 0.614 ± 0.014 & 0.732 ± 0.006 & 0.628 ± 0.006 & 0.774 ± 0.019 & 0.301 ± 0.012 & 0.345 ± 0.007 & 0.543 ± 0.016 & 0.972 ± 0.002 & 0.938 ± 0.002 & 0.7806 ± 0.0298 \\
Yi-1.5-9B-Chat & 0.488 ± 0.008 & 0.515 ± 0.014 & 0.649 ± 0.006 & 0.546 ± 0.006 & 0.774 ± 0.019 & 0.227 ± 0.011 & 0.330 ± 0.007 & 0.537 ± 0.016 & 0.985 ± 0.001 & 0.934 ± 0.002 & 0.7007 ± 0.0329 \\
%gemma-2-27b-it & 0.616 ± 0.008 & 0.669 ± 0.013 & 0.781 ± 0.006 & 0.670 ± 0.006 & 0.800 ± 0.018 & 0.222 ± 0.011 & 0.005 ± 0.001 &  0.536 ± 0.016 & 0.220 ± 0.004	& 0.331 ± 0.004 & 0.8163 ± 0.0278 \\
%gemma-2-9b-it & 0.566 ± 0.008 & 0.629 ± 0.014 & 0.745 ± 0.006 & 0.625 ± 0.006 & 0.766 ± 0.019 & 0.209 ± 0.011 & 0.221 ± 0.006 & 0.536 ± 0.016 & 0.230  ± 0.004 & 0.399  ± 0.005 & 0.7796 ± 0.0303 \\
\bottomrule
\end{tabular}
} 
\caption{Close-ended results.}
\label{tab:close_ended_benchmarks}
\end{table*}

\fi

==> latex/tables/open_ended_careqa.tex <==
\begin{table*}[h]
\centering
\renewcommand{\arraystretch}{1.5} 
\resizebox{2.1\columnwidth}{!}{%
\begin{tabular}{l|ccccccc}
\toprule
\textbf{Model} & \multicolumn{7}{c}{\textbf{Open-ended medical questions}} \\ 
& \multicolumn{7}{c}{\textbf{\careqa{}-Open}} \\
& \textbf{BERTScore $\uparrow$} & \textbf{BLEU $\uparrow$} & \textbf{BLEURT $\uparrow$} & \textbf{MoverScore $\uparrow$} & \textbf{ROUGE1 $\uparrow$} & \textbf{ROUGE2 $\uparrow$} & \textbf{ROUGEL $\uparrow$} \\  
\midrule
BioMistral-MedMNX & 0.835 ± 0.001 & 0.003 ± 0.000 & -1.040 ± 0.007 & 0.517 ± 0.001 & 0.069 ± 0.001 & 0.017 ± 0.001 & 0.057 ± 0.001 \\
JSL-MedLlama-3-8B-v2.0 & 0.844 ± 0.001 & 0.007 ± 0.001 & -0.908 ± 0.010 & 0.527 ± 0.001 & 0.083 ± 0.002 & 0.025 ± 0.001 & 0.070 ± 0.002 \\
Llama3-Med42-8B & 0.839 ± 0.001 & 0.005 ± 0.001 & -0.989 ± 0.012 & 0.521 ± 0.001 & 0.090 ± 0.003 & 0.022 ± 0.002 & 0.074 ± 0.002 \\
Meta-Llama-3.1-70B-Instruct & 0.843 ± 0.001 & 0.007 ± 0.001 & -0.969 ± 0.012 & 0.526 ± 0.001 & 0.134 ± 0.003 & 0.030 ± 0.002 & 0.113 ± 0.003 \\
Meta-Llama-3.1-8B-Instruct & 0.830 ± 0.001 & 0.003 ± 0.000 & -1.128 ± 0.007 & 0.514 ± 0.001 & 0.065 ± 0.001 & 0.017 ± 0.001 & 0.052 ± 0.001 \\
Mistral-7B-Instruct-v0.3 & 0.849 ± 0.002 & 0.006 ± 0.002 & -0.892 ± 0.023 & 0.529 ± 0.002 & 0.145 ± 0.007 & 0.038 ± 0.004 & 0.129 ± 0.006 \\
Mixtral-8x7B-Instruct-v0.1 & 0.814 ± 0.001 & 0.000 ± 0.000 & -1.264 ± 0.007 & 0.492 ± 0.001 & 0.051 ± 0.002 & 0.002 ± 0.000 & 0.045 ± 0.002 \\
Phi-3-medium-4k-instruct & 0.847 ± 0.001 & 0.008 ± 0.001 & -0.883 ± 0.013 & 0.529 ± 0.001 & 0.145 ± 0.003 & 0.034 ± 0.002 & 0.122 ± 0.003 \\
Phi-3-mini-4k-instruct & 0.839 ± 0.001 & 0.004 ± 0.001 & -0.986 ± 0.009 & 0.520 ± 0.001 & 0.115 ± 0.003 & 0.022 ± 0.001 & 0.097 ± 0.002 \\
Qwen2-7B-Instruct & 0.844 ± 0.001 & 0.006 ± 0.001 & -0.896 ± 0.009 & 0.527 ± 0.001 & 0.133 ± 0.003 & 0.028 ± 0.001 & 0.111 ± 0.002 \\
Yi-1.5-34B-Chat & 0.845 ± 0.001 & 0.008 ± 0.001 & -0.887 ± 0.009 & 0.526 ± 0.001 & 0.141 ± 0.003 & 0.034 ± 0.001 & 0.119 ± 0.002 \\
Yi-1.5-9B-Chat & 0.843 ± 0.000 & 0.007 ± 0.000 & -0.906 ± 0.007 & 0.525 ± 0.001 & 0.136 ± 0.002 & 0.030 ± 0.001 & 0.113 ± 0.002 \\
%gemma-2-27b-it	& 0.820 ± 0.003	& 0.000 ± 0.000	& -1.179 ± 0.020	& 0.500 ± 0.002	& 0.058 ± 0.007	& 0.000 ± 0.000	& 0.051 ± 0.006 \\
%gemma-2-9b-it	& 0.819 ± 0.001 & 0.000 ± 0.000 &	-1.167 ± 0.007 & 0.496 ± 0.001	& 0.050 ± 0.002	& 0.001 ± 0.000	& 0.045 ± 0.002 \\
\bottomrule
\end{tabular}
} 
\caption{Results for \careqa{}-Open \textcolor{red}{quitar}}
\label{tab:question_entailment_results}
\end{table*}

==> latex/tables/open_ended_medical_translation.tex <==
\begin{table*}[h]
\centering
\renewcommand{\arraystretch}{1.5} 
\resizebox{2.1\columnwidth}{!}{%
\begin{tabular}{l|ccccccc}
\toprule
\textbf{Model} & \multicolumn{6}{c}{\textbf{Medical Translation}} \\ 
& \multicolumn{6}{c}{\textbf{Med English to Spanish}}  \\
& \textbf{BLEU $\uparrow$} & \textbf{BLEURT $\uparrow$} & \textbf{MoverScore $\uparrow$} & \textbf{ROUGE1 $\uparrow$} & \textbf{ROUGE2 $\uparrow$} & \textbf{ROUGEL $\uparrow$} \\  
\midrule
BioMistral-MedMNX & 0.000 ± 0.000 & -1.233 ± 0.005 & nan ± nan & 0.037 ± 0.001 & 0.003 ± 0.000 & 0.032 ± 0.001 \\
JSL-MedLlama-3-8B-v2.0 & 0.000 ± 0.000 & -1.132 ± 0.005 & nan ± nan & 0.029 ± 0.001 & 0.002 ± 0.000 & 0.025 ± 0.001 \\
Llama3-Med42-8B & 0.000 ± 0.000 & -1.134 ± 0.006 & nan ± nan & 0.021 ± 0.001 & 0.001 ± 0.000 & 0.018 ± 0.001 \\
Meta-Llama-3.1-70B-Instruct & 0.000 ± 0.000 & -1.173 ± 0.005 & nan ± nan & 0.014 ± 0.001 & 0.001 ± 0.000 & 0.012 ± 0.001 \\
Meta-Llama-3.1-8B-Instruct & 0.000 ± 0.000 & -1.306 ± 0.005 & nan ± nan & 0.036 ± 0.001 & 0.003 ± 0.000 & 0.030 ± 0.001 \\
Mistral-7B-Instruct-v0.3 & 0.000 ± 0.000 & -0.824 ± 0.005 & nan ± nan & 0.104 ± 0.002 & 0.007 ± 0.000 & 0.087 ± 0.001 \\
Mixtral-8x7B-Instruct-v0.1 & 0.000  ± 0.000	& -0.888  ± 0.006	& nan  ± nan	& 0.097  ± 0.001	& 0.007  ± 0.000	&0.080  ± 0.001 \\
Phi-3-medium-4k-instruct & 0.000 ± 0.000 & -1.128 ± 0.005 & nan ± nan & 0.032 ± 0.001 & 0.002 ± 0.000 & 0.027 ± 0.001 \\
Phi-3-mini-4k-instruct & 0.000 ± 0.000 & -1.177 ± 0.005 & nan ± nan & 0.029 ± 0.001 & 0.002 ± 0.000 & 0.025 ± 0.001 \\
Qwen2-72B-Instruct & 0.000 ± 0.000 & -0.903 ± 0.006 & nan ± nan & 0.087 ± 0.002 & 0.007 ± 0.000 & 0.072 ± 0.001 \\
Qwen2-7B-Instruct & - & - & - & - & - & - \\
Yi-1.5-34B-Chat & 0.000 ± 0.000 & -1.099 ± 0.006 & nan ± nan & 0.047 ± 0.001 & 0.003 ± 0.000 & 0.040 ± 0.001 \\
Yi-1.5-9B-Chat & 0.000 ± 0.000 & -0.999 ± 0.005 & nan ± nan & 0.072 ± 0.001 & 0.006 ± 0.000 & 0.062 ± 0.001 \\
gemma-2-27b-it & 0.000 ± 0.000	& -1.169 ± 0.004	& nan ± nan & 0.005 ± 0.000	& 0.000 ± 0.000	& 0.005 ± 0.000 \\
gemma-2-9b-it & - & - & - & - & - & - \\
\bottomrule
\end{tabular}%
}
\caption{Medical Translation}
\label{tab:medical_translation}
\end{table*}

==> latex/tables/perplexity_clinical_note_taking_and_open_ended.tex <==
\begin{table*}[h]
\centering
\renewcommand{\arraystretch}{2} 
\resizebox{2\columnwidth}{!}{%
%\rotatebox{90}{
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\toprule
\textbf{Model} & \multicolumn{6}{c|}{\textbf{Clinical Note-taking}} & \multicolumn{6}{c}{\textbf{Open-ended Medical Questions}} \\
 & \multicolumn{3}{c|}{\textbf{ACI Bench}} & \multicolumn{3}{c|}{\textbf{MTS Dialog}} & \multicolumn{3}{c|}{\textbf{MedDialog Raw}} & \multicolumn{3}{c}{\textbf{MediQA2019}} \\
 & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$} & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$} & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$} & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$} \\
\midrule 
BioMistral-MedMNX & 0.601 & 1.517 & 13.894 & 1.059 & 2.083 & 132.827 & 1.043 & 2.060 & 74.760 & 0.416 & 1.335 & 6.044 \\
JSL-MedLlama-3-8B-v2.0 & 0.703 & 1.628 & 21.725 & 1.099 & 2.143 & 160.188 & 1.179 & 2.265 & 131.509 & 0.517 & 1.431 & 9.312 \\
Llama3-Med42-8B & 0.485 & 1.399 & 8.357 & 1.060 & 2.085 & 133.416 & 1.069 & 2.097 & 83.115 & 0.405 & 1.324 & 5.754 \\
Meta-Llama-3.1-70B-Instruct & - & - & - & 0.984 & 1.978 & 93.943 & 0.993 & 1.991 & 60.907 & 0.245 & 1.185 & 2.886 \\
Meta-Llama-3.1-8B-Instruct & 0.612 & 1.529 & 14.618 & 1.074 & 2.105 & 142.211 & 1.060 & 2.085 & 80.124 & 0.430 & 1.347 & 6.407 \\
Mistral-7B-Instruct-v0.3 & 0.596 & 1.512 & 13.628 & 1.053 & 2.074 & 129.076 & 1.073 & 2.104 & 84.603 & 0.420 & 1.338 & 6.145 \\
Mixtral-8x7B-Instruct-v0.1 & 0.566 & 1.481 & 11.933 & 1.046 & 2.064 & 125.070 & 1.028 & 2.039 & 70.258 & 0.300 & 1.232 & 3.662 \\
Phi-3-medium-4k-instruct & 0.642 & 1.560 & 16.600 & 0.971 & 1.960 & 88.447 & 1.068 & 2.097 & 82.957 & 0.410 & 1.329 & 5.884 \\
Phi-3-mini-4k-instruct & 0.599 & 1.514 & 13.754 & 0.972 & 1.962 & 89.163 & 1.082 & 2.117 & 87.936 & 0.444 & 1.360 & 6.796 \\
%Qwen2-72B-Instruct & - & - & - & 0.954 & 1.938 & 82.027 & 0.938 & 1.916 & 48.395 & 0.350 & 1.274 & 4.533 \\
Qwen2-7B-Instruct & 0.619 & 1.535 & 15.009 & 1.063 & 2.089 & 135.111 & 1.044 & 2.063 & 75.218 & 0.447 & 1.363 & 6.895 \\
Yi-1.5-34B-Chat & 0.728 & 1.657 & 24.270 & 1.099 & 2.143 & 160.265 & 1.101 & 2.145 & 95.042 & 0.485 & 1.399 & 8.112 \\
Yi-1.5-9B-Chat & 0.711 & 1.636 & 22.456 & 1.180 & 2.265 & 232.073 & 1.123 & 2.178 & 104.205 & 0.532 & 1.446 & 9.968 \\
%gemma-2-27b-it & - &- & -& -& -&- & - & - & - & -& -&-\\
%gemma-2-9b-it & - & - & - & - &  - & & 3.647 & 12.528 & 3563621.691 & 3.400& 10.555 & - \\

\bottomrule
\end{tabular}%
}
%}
\caption{Perplexity results for Open-ended Medical Questions.}
\end{table*}

==> latex/tables/perplexity_open_ended_old.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.5} 
\resizebox{2\columnwidth}{!}{%
%\rotatebox{90}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
\textbf{Model} & \multicolumn{9}{c}{\textbf{Open-ended Medical Questions}} \\
 & \multicolumn{3}{c|}{\textbf{\careqa{}-Open}} & \multicolumn{3}{c|}{\textbf{MedDialog Raw}} & \multicolumn{3}{c}{\textbf{MediQA2019}} \\
 & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$} & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$} & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$}\\
\midrule 
BioMistral-MedMNX & 1.385 & 2.612 & 688.279 & 1.043 & 2.060 & 74.760 & 0.416 & 1.335 & 6.044 \\
JSL-MedLlama-3-8B-v2.0 & 1.761 & 3.389 & 4050.635 & 1.179 & 2.265 & 131.509 & 0.517 & 1.431 & 9.312 \\
Llama3-Med42-8B & 1.331 & 2.516 & 534.246 & 1.069 & 2.097 & 83.115 & 0.405 & 1.324 & 5.754 \\

Meta-Llama-3.1-70B-Instruct & 1.274 & 2.418 & 406.877 & 0.993 & 1.991 & 60.907 & 0.245 & 1.185 & 2.886 \\
Meta-Llama-3.1-8B-Instruct & 1.346 & 2.543 & 573.612 & 1.060 & 2.085 & 80.124 & 0.430 & 1.347 & 6.407 \\
Mistral-7B-Instruct-v0.3 & 1.411 & 2.659 & 777.203 & 1.073 & 2.104 & 84.603 & 0.420 & 1.338 & 6.145 \\
Mixtral-8x7B-Instruct-v0.1 & 4.405 & 21.184 & nan & 1.028 & 2.039 & 70.258 & 0.300 & 1.232 & 3.662 \\
Phi-3-medium-4k-instruct & 1.298 & 2.458 & 455.98 & 1.068 & 2.097 & 82.957 & 0.410 & 1.329 & 5.884 \\
Phi-3-mini-4k-instruct & 1.299 & 2.460 & 458.481 & 1.082 & 2.117 & 87.936 & 0.444 & 1.360 & 6.796 \\
Qwen2-7B-Instruct & 1.438 & 2.710 & 885.33 & 1.044 & 2.063 & 75.218 & 0.447 & 1.363 & 6.895 \\
Yi-1.5-34B-Chat & 1.512 & 2.852 & 1254.136 & 1.101 & 2.145 & 95.042 & 0.485 & 1.399 & 8.112 \\
Yi-1.5-9B-Chat & 1.603 & 3.037 & 1921.553 & 1.123 & 2.178 & 104.205 & 0.532 & 1.446 & 9.968 \\
%gemma-2-27b-it & 8.600 & 388.080 & 417929466779407872.000 & & & & 7.230	& 150.161	& 36615253021450.047 \\
%gemma-2-9b-it & 3.908 & 15.009 & 101542723.787 & 3.647 & 12.528 & 3563621.691 & 3.400 & 10.555 & 2387337.872 \\

\bottomrule
\end{tabular}%
}
%}
\caption{Perplexity results for Open-ended Medical Questions.}
\end{table*}


==> latex/tables/perplexity_table.tex <==
\begin{table*}[h]
\centering
\renewcommand{\arraystretch}{1.5} 
\resizebox{2.2\columnwidth}{!}{%
%\rotatebox{90}{
\begin{tabular}{l|ccc|ccc|ccc|ccc|ccc}
\toprule
\textbf{Model} & \multicolumn{6}{c|}{\textbf{Clinical Note-taking}} & \multicolumn{3}{c|}{\textbf{Open-ended Medical Questions}} & \multicolumn{3}{c|}{\textbf{Question Entailment}} & \multicolumn{3}{c}{\textbf{Summarization}} \\
 & \multicolumn{3}{c|}{\textbf{ACI Bench}} & \multicolumn{3}{c|}{\textbf{MTS Dialog}} & \multicolumn{3}{c|}{\textbf{MedDialog Raw}} & \multicolumn{3}{c|}{\textbf{MedDialog Qsumm}} & \multicolumn{3}{c}{\textbf{Mimic-III}} \\
 & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$} & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$} & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$} & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$} & \textbf{Bits per Byte $\downarrow$} & \textbf{Byte Perplexity $\downarrow$} & \textbf{Word Perplexity $\downarrow$} \\
\midrule 
BioMistral-MedMNX & 601 & 1517 & 13894 & 1059 & 2083 & 132827 & 1043 & 2060 & 74760 & 1471 & 2772 & 275846 & 1771 & 3413 & 4697580 \\
JSL-MedLlama-3-8B-v2.0 & 703 & 1628 & 21725 & 1099 & 2143 & 160188 & 1179 & 2265 & 131509 & 1715 & 3282 & 699785 & 2035 & 4099 & 16607943 \\
Llama3-Med42-8B & 485 & 1399 & 8357 & 1060 & 2085 & 133416 & 1069 & 2097 & 83115 & 1359 & 2564 & 179527 & 1839 & 3577 & 6489224 \\
Meta-Llama-3.1-70B-Instruct &  &  &  & 984 & 1978 & 93943 & 993 & 1991 & 60907 & 1280 & 2428 & 132988 &  &  &  \\
Meta-Llama-3.1-8B-Instruct & 612 & 1529 & 14618 & 1074 & 2105 & 142211 & 1060 & 2085 & 80124 & 1371 & 2587 & 188513 & 1826 & 3545 & 6106099 \\
Mistral-7B-Instruct-v0.3 & 596 & 1512 & 13628 & 1053 & 2074 & 129076 & 1073 & 2104 & 84603 & 1447 & 2727 & 251938 & 1790 & 3457 & 5138524 \\
Mixtral-8x7B-Instruct-v0.1 & 566	& 1481	& 11933	& 1046	& 2064	& 125070	& 1028	& 2039	& 70258	& 1370	& 2586	& 187912	& 1679	& 3202	& 3028534 \\
Phi-3-medium-4k-instruct & 642 & 1560 & 16600 & 971 & 1960 & 88447 & 1068 & 2097 & 82957 & 1332 & 2517 & 162163 & 2084 & 4239 & 20901351 \\
Phi-3-mini-4k-instruct & 599 & 1514 & 13754 & 972 & 1962 & 89163 & 1082 & 2117 & 87936 & 1311 & 2481 & 149718 & 1902 & 3737 & 8784663 \\
Qwen2-72B-Instruct &  &  &  & 954 & 1938 & 82027 & 938 & 1916 & 48395 & 1283 & 2433 & 134531 &  &  &  \\
Qwen2-7B-Instruct & 619 & 1535 & 15009 & 1063 & 2089 & 135111 & 1044 & 2063 & 75218 & 1383 & 2608 & 197167 & 1878 & 3676 & 7839132 \\
Yi-1.5-34B-Chat &  &  &  & 1099 & 2143 & 160265 & 1101 & 2145 & 95042 & 1437 & 2708 & 242427 &  &  &  \\
Yi-1.5-9B-Chat &  
711	& 1636	& 22456 & 1180 & 2265 & 232073 & 1123 & 2178 & 104205 & 1470 & 2771 & 275222 & 2341 & 5067 & 71436330 \\
\bottomrule
\end{tabular}%
}
%}
\caption{Perplexity results}
\end{table*}

==> latex/tables/prometheus_1.tex <==
\begin{table*}[H]
\centering
\renewcommand{\arraystretch}{1.5} 
\resizebox{2\columnwidth}{!}{%
%\rotatebox{90}{
\begin{tabular}{l|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Treatment recommendations} & \textbf{Question Entailment} & \textbf{Summarization} & \multicolumn{2}{c|}{\textbf{Clinical Note-Taking}}\\
 & \textbf{MedText} & \textbf{MedDialog Qsumm} & \textbf{Mimic-III} & \textbf{ACI Bench} & \textbf{MTS Dialog} \\
& \multicolumn{5}{c}{\textbf{Prometheus $\uparrow$}}\\
\midrule 
BioMistral-MedMNX           & 0.225 ± 0.063 & 0.163 ± 0.005 & 0.330 ± 0.016 & 0.273 ± 0.027 & 0.297 ± 0.009  \\
JSL-MedLlama-3-8B-v2.0      & 0.263 ± 0.084 & 0.087 ± 0.004 & 0.298 ± 0.017 & 0.365 ± 0.031 & 0.172 ± 0.008 \\
Llama3-Med42-8B             & 0.138 ± 0.062 & 0.241 ± 0.007 & 0.213 ± 0.016 & 0.157 ± 0.024 & 0.130 ± 0.008 \\
Meta-Llama-3.1-70B-Instruct  & 0.062 ± 0.043 & 0.314 ± 0.007 & 0.342 ± 0.016 & 0.313 ± 0.026 & 0.281 ± 0.009 \\
Meta-Llama-3.1-8B-Instruct   & 0.188 ± 0.063 & 0.156 ± 0.005 & 0.263 ± 0.015 & 0.245 ± 0.027 & 0.237 ± 0.008  \\
Mistral-7B-Instruct-v0.3     & 0.050 ± 0.029 & 0.194 ± 0.006 & 0.187 ± 0.015 & 0.087 ± 0.018 & 0.055 ± 0.005 \\
Mixtral-8x7B-Instruct-v0.1   & 0.075 ± 0.036 & 0.112 ± 0.005 & 0.252 ± 0.016 & 0.090 ± 0.017 & 0.198 ± 0.009 \\
Phi-3-medium-4k-instruct     & 0.175 ± 0.064 & 0.168 ± 0.005 & 0.358 ± 0.017 & 0.190 ± 0.023 & 0.219 ± 0.008  \\
Phi-3-mini-4k-instruct       & 0.125 ± 0.057 & 0.126 ± 0.005 & 0.376 ± 0.016 & 0.287 ± 0.027 & 0.280 ± 0.009 \\
%Qwen2-72B-Instruct           & -            & 0.260 ± 0.006 & -            & 0.332 ± 0.026 & -            & -            & -            \\
Qwen2-7B-Instruct            & 0.125 ± 0.052 & 0.177 ± 0.006 & 0.267 ± 0.014 & 0.255 ± 0.026 & 0.144 ± 0.007  \\
Yi-1.5-34B-Chat              & 0.287 ± 0.069 & 0.179 ± 0.006 & 0.372 ± 0.016 & 0.342 ± 0.030 & 0.420 ± 0.008  \\
Yi-1.5-9B-Chat               & 0.138 ± 0.067 & 0.405 ± 0.007            & 0.550 ± 0.015 & 0.362 ± 0.026 & 0.397 ± 0.008 \\
%gemma-2-27b-it               & 0.000 ± 0.000 & 0.001 ± 0.000 & 0.002 ± 0.001 & 0.000 ± 0.000 & 0.000 ± 0.000  \\
%gemma-2-9b-it                & 0.000 ± 0.000 & 0.002 ± 0.001 & 0.011 ± 0.004 & 0.000 ± 0.000 & 0.000 ± 0.000 \\

\bottomrule
\end{tabular}%
}
%}
\caption{Prometheus results for the following tasks: making diagnosis and treatment recommendations, question entailment, summarization and clinical note-taking.
}
\end{table*}

==> latex/tables/prometheus_2.tex <==
\begin{table*}[H]
\centering
\renewcommand{\arraystretch}{1.7} 
\resizebox{1\columnwidth}{!}{%
%\rotatebox{90}{
\begin{tabular}{l|c|c|c}
\toprule
\textbf{Model} & \multicolumn{3}{c}{\textbf{Open-ended Medical Questions}} & \textbf{Medical Factuality}  \\
& \textbf{MedDialog Raw} & \textbf{MediQA2019} & \textbf{\careqa{}-Open}\\% & \textbf{OLAPH}\\
& \multicolumn{3}{c}{\textbf{Prometheus $\uparrow$}}\\
\midrule 
BioMistral-MedMNX  &0.535 ± 0.005 & 0.342 ± 0.007 & 0.272 ± 0.006\\
JSL-MedLlama-3-8B-v2.0   & 0.304 ± 0.005 & 0.459 ± 0.008 & 0.307 ± 0.007\\
Llama3-Med42-8B             & 0.138 ± 0.062 & 0.241 ± 0.007 & 0.230 ± 0.006\\
Meta-Llama-3.1-70B-Instruct  &  0.293 ± 0.005 & 0.326 ± 0.008 & 0.296 ± 0.006 \\
Meta-Llama-3.1-8B-Instruct   & 0.375 ± 0.005 & 0.229 ± 0.007 & 0.225 ± 0.006\\
Mistral-7B-Instruct-v0.3  & 0.476 ± 0.005 & 0.384 ± 0.008 & 0.087 ± 0.004 \\
Mixtral-8x7B-Instruct-v0.1   & 0.543 ± 0.005 & 0.361 ± 0.008 & 0.030 ± 0.002 \\
Phi-3-medium-4k-instruct  & 0.249 ± 0.005 & 0.281 ± 0.008 & 0.308 ± 0.007\\
Phi-3-mini-4k-instruct & 0.353 ± 0.005 & 0.328 ± 0.008 & 0.299 ± 0.006\\
%Qwen2-72B-Instruct           & -            & 0.260 ± 0.006 & -            & 0.332 ± 0.026 & -            & -            & -            \\
Qwen2-7B-Instruct   & 0.541 ± 0.005 & 0.267 ± 0.007 & 0.427 ± 0.007\\
Yi-1.5-34B-Chat & 0.508 ± 0.005 & 0.347 ± 0.009 & 0.488 ± 0.007 \\
Yi-1.5-9B-Chat & 0.288 ± 0.005 & 0.417 ± 0.009 & 0.612 ± 0.006 \\
%gemma-2-27b-it  & 0.001 ± 0.000 & 0.000 ± 0.000 & 0.003 ± 0.001\\
%gemma-2-9b-it & 0.002 ± 0.000 & 0.003 ± 0.001 & 0.006 ± 0.001\\

\bottomrule
\end{tabular}%
}
%}
\caption{Prometheus results for the open-ended medical questions.% and medical factuality.
}
\end{table*}


==> latex/tables/table6.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{rcl}
\multicolumn{3}{c}{{\color[HTML]{000000} \Large \textsc{Open-ended}\vspace{4pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
{\color[HTML]{000000} \textbf{\large \textsc{Tasks}}}                                                                       & {\color[HTML]{000000} \textbf{\large \textsc{Metrics}}}                                                                                  & {\color[HTML]{000000} \textbf{\large \textsc{Datasets}}}                                                                                                                                                                                                                                                                 \\ \hline
\vspace{2pt}
\rowcolor[HTML]{EFEFD2} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Multiple choice\\ questions\end{tabular}}}   & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· MedMCQA \cite{pmlr-v174-pal22a}\\ · PubMedQA \cite{jin2019pubmedqa}\\ · MedQA \cite{jin2020disease}\\ · MMLU \cite{hendrycks2020measuring}\\ · CareQA\end{tabular}}                                                                                   \\
\rowcolor[HTML]{E3EFD6} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Prescriptions \\ writing \end{tabular}}}            & {\color[HTML]{656565} "}                                                                                          & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/devlocalhost/prescription-full}{Prescription} \vspace{2pt}}                                                                                                                                                                                \\

\rowcolor[HTML]{C8E9D9} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ classification\end{tabular}}}      & {\color[HTML]{656565} "}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://www.kaggle.com/datasets/chaitanyakck/medical-text/data}{Medical Text for classification} \cite{10.1145/3582768.3582795}\\ · \href{https://www.kaggle.com/datasets/tboyle10/medicaltranscriptions}{Medical Transcriptions}\end{tabular}\vspace{2pt}} \\



\rowcolor[HTML]{CDEBEB} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Relation\\ extraction\end{tabular}}}              & {\color[HTML]{656565} "}                                                                                          & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/YufeiHFUT/BioRED_all_info}{BioRED} \cite{luo2022biored}}         \\

\hline
\multicolumn{3}{l}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\
\multicolumn{3}{c}{{\color[HTML]{000000} \large \textsc{Close-ended}\vspace{4pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline

\rowcolor[HTML]{C7DBE9} 
        
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Open-ended\\ medical questions\end{tabular}}}     & {\color[HTML]{656565} \normalsize \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT, ROUGE,\\ BERTScore, MoverScore, \\ Prometheus, Perplexity \end{tabular}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://huggingface.co/datasets/bigbio/meddialog}{MedDialog} \cite{zeng2020meddialog} \\ · \href{https://huggingface.co/datasets/bigbio/mediqa_qa}{MEDIQA2019} \cite{MEDIQA2019} \end{tabular}\vspace{2pt}}  


\\


\rowcolor[HTML]{E1DEE9} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Making diagnosis \\ and treatment\\ recommendations\end{tabular}}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT, ROUGE,\\ BERTScore, MoverScore\\ Prometheus, Perplexity\end{tabular}}  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/BI55/MedText}{MedText} \vspace{2pt}}                                                                                                                                                                                                       \\
\rowcolor[HTML]{E5CFDF} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Clinical\\ note-taking\end{tabular}}}             & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT, ROUGE,\\ BERTScore, MoverScore,\\ Prometheus, Perplexity\end{tabular}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://huggingface.co/datasets/har1/MTS_Dialogue-Clinical_Note}{MTS-Dialog} \cite{mts-dialog}\\ · ACI-Bench \cite{aci-bench}\end{tabular} \vspace{2pt}}                                                                                                     \\ 


\rowcolor[HTML]{EFD6DC} 
{\color[HTML]{656565} \textbf{Summarization}}                                                              & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT, ROUGE,\\ BERTScore, MoverScore,\\ Perplexity, F1-RadGraph\end{tabular}} & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/dmacres/mimiciii-hospitalcourse-meta}{MIMIC-III} \cite{johnson2016mimic}\vspace{2pt}}                                                                                                                                                      \\

\rowcolor[HTML]{EFD6DC} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Question\\ entailment\end{tabular}}}              & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT, ROUGE,\\ BERTScore, MoverScore,\\ Prometheus, Perplexity\end{tabular}}  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/lighteval/med_dialog}{Meddialog} \cite{zeng2020meddialog} \vspace{2pt}}                                                                                                                                                                                                                        \\
%\rowcolor[HTML]{EFD6DC} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ translation\end{tabular}}}         & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore\end{tabular}}              & {\color[HTML]{656565} · 
%\href{https://huggingface.co/datasets/ayoubkirouane/med_en2es}{Med\_English2Spanish} \vspace{2pt}}                                                                                                                                                          \\

%\rowcolor[HTML]{E9E1DE} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ classification\end{tabular}}}      & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://www.kaggle.com/datasets/chaitanyakck/medical-text/data}{Medical Text for classification} \cite{10.1145/3582768.3582795}\\ · \href{https://www.kaggle.com/datasets/tboyle10/medicaltranscriptions}{Medical Transcriptions}\end{tabular}} \\
%\rowcolor[HTML]{D7CCC7} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Information\\ extraction\end{tabular}}}           & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}Exact maching\\ F1-Score\end{tabular}}                                  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/rajpurkar/squad_v2/viewer/squad_v2/validation?p=52}{SQuAD} \cite{rajpurkar2018know} \vspace{2pt}}                                                                                                                                          \\
 \hline
\end{tabular}%
} \caption{This table presents the tasks evaluated in this paper, listed in different rows. The second column details the metrics used for each task, including Bits per Byte, Byte Perplexity, and Word Perplexity for perplexity measurements. The third column outlines the different benchmarks used for each task.
} \label{tab:tasks_bench_metrics}
\end{table*}

==> latex/tables/table_10.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[t]
\centering
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{rcl}
\multicolumn{3}{c}{{\color[HTML]{000000} \Large \textsc{Close-ended}\vspace{4pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
{\color[HTML]{000000} \textbf{\large \textsc{Tasks}}}                                                                       & {\color[HTML]{000000} \textbf{\large \textsc{Metrics}}}                                                                                  & {\color[HTML]{000000} \textbf{\large \textsc{Datasets}}}                                                                                                                                                                                                                                                                 \\ \hline
\vspace{2pt}
\rowcolor[HTML]{EFEFD2} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Multiple choice\\ questions\end{tabular}}}   & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· MedMCQA \cite{pmlr-v174-pal22a}\\ · PubMedQA \cite{jin2019pubmedqa}\\ · MedQA \cite{jin2020disease}\\ · MMLU \cite{hendrycks2020measuring}\\ · \careqa{}-close\end{tabular}}                                                                                   \\
\rowcolor[HTML]{E3EFD6} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Prescriptions \\ writing \end{tabular}}}            & {\color[HTML]{656565} "}                                                                                          & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/devlocalhost/prescription-full}{Prescription} \vspace{2pt}}                                                                                                                                                                                \\

\rowcolor[HTML]{C8E9D9} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ classification\end{tabular}}}      & {\color[HTML]{656565} "}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://www.kaggle.com/datasets/chaitanyakck/medical-text/data}{Medical Text for classification} \cite{10.1145/3582768.3582795}\\ · \href{https://www.kaggle.com/datasets/tboyle10/medicaltranscriptions}{Medical Transcriptions}\end{tabular}\vspace{2pt}} \\



\rowcolor[HTML]{CDEBEB} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Relation\\ extraction\end{tabular}}}              & {\color[HTML]{656565} "}                                                                                          & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/YufeiHFUT/BioRED_all_info}{BioRED} \cite{luo2022biored}}         \\

\hline
\multicolumn{3}{l}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\
\multicolumn{3}{c}{{\color[HTML]{000000} \Large \textsc{Open-ended}\vspace{4pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline

\rowcolor[HTML]{C7DBE9} 
        
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Open-ended\\ medical questions\end{tabular}}}     & {\color[HTML]{656565} \normalsize \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT, ROUGE,\\ BERTScore, MoverScore,\\ Prometheus, Perplexity\end{tabular}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://huggingface.co/datasets/bigbio/meddialog}{MedDialog Raw} \cite{zeng2020meddialog} \\ · \href{https://huggingface.co/datasets/bigbio/mediqa_qa}{MEDIQA2019} \cite{MEDIQA2019} \\· \careqa{}-open 
\end{tabular}\vspace{2pt}}  


\\


\rowcolor[HTML]{E1DEE9} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Making diagnosis \\ and treatment\\ recommendations\end{tabular}}} & {\color[HTML]{656565} " }  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/BI55/MedText}{MedText} \vspace{2pt}}                                                                                                                                                                                                       \\
\rowcolor[HTML]{E5CFDF} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Clinical\\ note-taking\end{tabular}}}             & {\color[HTML]{656565} " } & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://huggingface.co/datasets/har1/MTS_Dialogue-Clinical_Note}{MTS-Dialog} \cite{mts-dialog}\\ · ACI-Bench \cite{aci-bench}\end{tabular} \vspace{2pt}}                                                                                                     \\ 


\rowcolor[HTML]{EFD6DC} 
{\color[HTML]{656565} \textbf{Summarization}}                                                              & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}} " \\ + F1-RadGraph \end{tabular}} & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/dmacres/mimiciii-hospitalcourse-meta}{MIMIC-III} \cite{johnson2016mimic}\vspace{2pt}}                                                                                                                                                      \\

\rowcolor[HTML]{EFD6DC} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Question\\ entailment\end{tabular}}}              & {\color[HTML]{656565} "}  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/lighteval/med_dialog}{Meddialog Qsumm} \cite{zeng2020meddialog} }                                                                                                                                                                                                                        \\
%\rowcolor[HTML]{EFD6DC} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ translation\end{tabular}}}         & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore\end{tabular}}              & {\color[HTML]{656565} · 
%\href{https://huggingface.co/datasets/ayoubkirouane/med_en2es}{Med\_English2Spanish} \vspace{2pt}}                                                                                                                                                          \\

%\rowcolor[HTML]{E9E1DE} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ classification\end{tabular}}}      & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://www.kaggle.com/datasets/chaitanyakck/medical-text/data}{Medical Text for classification} \cite{10.1145/3582768.3582795}\\ · \href{https://www.kaggle.com/datasets/tboyle10/medicaltranscriptions}{Medical Transcriptions}\end{tabular}} \\
%\rowcolor[HTML]{D7CCC7} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Information\\ extraction\end{tabular}}}           & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}Exact maching\\ F1-Score\end{tabular}}                                  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/rajpurkar/squad_v2/viewer/squad_v2/validation?p=52}{SQuAD} \cite{rajpurkar2018know} \vspace{2pt}}                                                                                                                                          \\
 \hline
\end{tabular}%
} \caption{This table presents the tasks implemented in this paper, listed in different rows. The first column specifies the different tasks. The second details the metrics used for each task, Perplexity includes Bits per Byte, Byte Perplexity, and Word Perplexity. The third column outlines the different benchmarks used for each task.
} \label{tab:tasks_bench_metrics}
\end{table*}

==> latex/tables/tasks_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{rcl}
\hline
\multicolumn{3}{c}{{\color[HTML]{000000} \textsc{Healthcare}\vspace{5pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ \hline
{\color[HTML]{000000} \textbf{Task}}                                                                       & {\color[HTML]{000000} \textbf{Metrics}}                                                                                               & {\color[HTML]{000000} \textbf{Datasets}}                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{EFEFD2} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Closed-ended\\ medical questions\end{tabular}}}   & {\color[HTML]{656565} Accuracy}                                                                                                       & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· MedMCQA \cite{pmlr-v174-pal22a}\\ · PubMedQA \cite{jin2019pubmedqa}\\ · MedQA \cite{jin2020disease}\\ · MMLU \cite{hendrycks2020measuring}\\ · CareQA \vspace{5pt}\end{tabular}}                                                                                                                                                                                            \\
\rowcolor[HTML]{E3EFD6} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Open-ended\\ medical questions\end{tabular}}}     & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore \\ MoverScore, Prometheus \vspace{5pt}\end{tabular}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· Meddialog \cite{zeng2020meddialog}\\ HuggingFace (\href{https://huggingface.co/datasets/bigbio/meddialog}{bigbio/meddialog})\end{tabular}}                                                                                                                                                                                                                                  \\
\rowcolor[HTML]{C8E9D9} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Making treatment\\ recommendations\end{tabular}}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore, Prometheus \vspace{5pt}\end{tabular}}  & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· MedText\\ HuggingFace (\href{https://huggingface.co/datasets/BI55/MedText}{BI55/MedText})\end{tabular}}                                                                                                                                                                                                                                                                     \\
\rowcolor[HTML]{CDEBEB} 
{\color[HTML]{656565} \textbf{Writing prescriptions}}                                                      & {\color[HTML]{656565} Accuracy}                                                                                                       & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· Prescription \\ HuggingFace (\href{https://huggingface.co/datasets/devlocalhost/prescription-full}{devlocalhost/prescription-full})\end{tabular}}                                                                                                                                                                                                                           \\
\rowcolor[HTML]{C7DBE9} 
{\color[HTML]{656565} \textbf{Clinical note-taking}}                                                       & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\  MoverScore, Prometheus \vspace{5pt}\end{tabular}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· MTS-Dialog \cite{mts-dialog}\\ HuggingFace (\href{https://huggingface.co/datasets/har1/MTS_Dialogue-Clinical_Note}{har1/MTS_Dialogue-Clinical_Note}\\ · ACI-Bench \cite{aci-bench}\end{tabular}}                                                                                                                                                                            \\
\multicolumn{3}{l}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\
\multicolumn{3}{c}{{\color[HTML]{656565} \textsc{NLP}\vspace{5pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\rowcolor[HTML]{E1DEE9} 
{\color[HTML]{656565} \textbf{Summarization}}                                                              & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore, F1-RadGraph \vspace{5pt}\end{tabular}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· MIMIC-III \cite{johnson2016mimic}\\ HuggingFace (\href{https://huggingface.co/datasets/dmacres/mimiciii-hospitalcourse-meta}{dmacres/mimiciii-hospitalcourse-meta}\end{tabular}}                                                                                                                                                                                            \\
\rowcolor[HTML]{DACEDE} 
{\color[HTML]{656565} \textbf{Question entailment}}                                                        & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore, Prometheus \vspace{5pt}\end{tabular}}  & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· Meddialog \cite{zeng2020meddialog} \\ HuggingFace (\href{https://huggingface.co/datasets/lighteval/med_dialog/discussions}{lighteval/med\_dialog})\end{tabular}}                                                                                                                                                                                                            \\
\rowcolor[HTML]{E5CFDF} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ translation\end{tabular}}}         & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore \vspace{5pt}\end{tabular}}              & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· ELRC-Medical-V2 \cite{losch2018european}\\ HuggingFace (\href{https://huggingface.co/datasets/qanastek/ELRC-Medical-V2}{qanastek/ELRC-Medical-V2}) \vspace{5pt}\end{tabular}}                                                                                                                                                                                               \\
\rowcolor[HTML]{EFD6DC} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ classification\end{tabular}}}      & {\color[HTML]{656565} Accuracy}                                                                                                       & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· Medical Text for classification \cite{10.1145/3582768.3582795}\\ Kaggle (\href{https://www.kaggle.com/datasets/chaitanyakck/medical-text/data}{Medical Text})\\ · Medical Transcriptions \href{https://www.mtsamples.com/}{mtsamples.com}\\ Kaggle (\href{https://www.kaggle.com/datasets/tboyle10/medicaltranscriptions}{Medical Transcriptions}\vspace{5pt}\end{tabular}} \\
\rowcolor[HTML]{E9E1DE} 
{\color[HTML]{656565} \textbf{Information extraction}}                                                     & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}Exact maching\\ F1-Score\end{tabular}}                                               & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· SQuAD \cite{rajpurkar2018know}\\ HuggingFace (\href{https://huggingface.co/datasets/rajpurkar/squad_v2/viewer/squad_v2/validation?p=52}{rajpurkar/squad_v2} \vspace{5pt}\end{tabular}}                                                                                                                                                                                      \\
\rowcolor[HTML]{E4D9D4} 
{\color[HTML]{656565} \textbf{Relation extraction}}                                                        & {\color[HTML]{656565} Accuracy}                                                                                                       & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· BioRED \cite{luo2022biored}\\ HuggingFace (\href{https://huggingface.co/datasets/YufeiHFUT/BioRED_all_info}{YufeiHFUT/BioRED\_all\_info}) \vspace{5pt}\end{tabular}}                                                                                                                                                                                                        \\ \hline
\end{tabular}%
}
\end{table*}

==> latex/tables/tasks_table_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{rcl}
\multicolumn{3}{c}{{\color[HTML]{000000} \Large \textsc{Healthcare}\vspace{4pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
{\color[HTML]{000000} \textbf{\large \textsc{Tasks}}}                                                                       & {\color[HTML]{000000} \textbf{\large \textsc{Metrics}}}                                                                                  & {\color[HTML]{000000} \textbf{\large \textsc{Datasets}}}                                                                                                                                                                                                                                                                 \\ \hline
\vspace{2pt}
\rowcolor[HTML]{EFEFD2} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Closed-ended\\ medical questions\end{tabular}}}   & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· MedMCQA \cite{pmlr-v174-pal22a}\\ · PubMedQA \cite{jin2019pubmedqa}\\ · MedQA \cite{jin2020disease}\\ · MMLU \cite{hendrycks2020measuring}\\ · CareQA\end{tabular}}                                                                                   \\
\rowcolor[HTML]{E3EFD6} 
        
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Open-ended\\ medical questions\end{tabular}}}     & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore \\ MoverScore, Prometheus\end{tabular}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://huggingface.co/datasets/bigbio/meddialog}{MedDialog} \cite{zeng2020meddialog} \\ · \href{https://huggingface.co/datasets/bigbio/mediqa_qa}{MEDIQA2019} \cite{MEDIQA2019} \end{tabular}\vspace{2pt}}  


\\
\rowcolor[HTML]{C8E9D9} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Making treatment\\ recommendations\end{tabular}}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore, Prometheus\end{tabular}}  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/BI55/MedText}{MedText} \vspace{2pt}}                                                                                                                                                                                                       \\
\rowcolor[HTML]{CDEBEB} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Writing\\ prescriptions\end{tabular}}}            & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/devlocalhost/prescription-full}{Prescription} \vspace{2pt}}                                                                                                                                                                                \\
\rowcolor[HTML]{C7DBE9} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Clinical\\ note-taking\end{tabular}}}             & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\  MoverScore, Prometheus\end{tabular}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://huggingface.co/datasets/har1/MTS_Dialogue-Clinical_Note}{MTS-Dialog} \cite{mts-dialog}\\ · ACI-Bench \cite{aci-bench}\end{tabular}}                                                                                                     \\ \hline
\multicolumn{3}{l}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\
\multicolumn{3}{c}{{\color[HTML]{000000} \large \textsc{NLP}\vspace{4pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\rowcolor[HTML]{E1DEE9} 
{\color[HTML]{656565} \textbf{Summarization}}                                                              & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore, F1-RadGraph\end{tabular}} & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/dmacres/mimiciii-hospitalcourse-meta}{MIMIC-III} \cite{johnson2016mimic}\vspace{2pt}}                                                                                                                                                      \\

\rowcolor[HTML]{DACEDE} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Question\\ entailment\end{tabular}}}              & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore, Prometheus\end{tabular}}  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/lighteval/med_dialog}{Meddialog} \cite{zeng2020meddialog} \vspace{2pt}}                                                                                                                                                                                                                        \\
\rowcolor[HTML]{E5CFDF} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ translation\end{tabular}}}         & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore\end{tabular}}              & {\color[HTML]{656565} · 


\href{https://huggingface.co/datasets/ayoubkirouane/med_en2es}{Med\_English2Spanish} \vspace{2pt}}                                                                                                                                                          \\
\vspace{2pt}

\rowcolor[HTML]{EFD6DC} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ classification\end{tabular}}}      & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://www.kaggle.com/datasets/chaitanyakck/medical-text/data}{Medical Text for classification} \cite{10.1145/3582768.3582795}\\ · \href{https://www.kaggle.com/datasets/tboyle10/medicaltranscriptions}{Medical Transcriptions}\end{tabular}} \\
\rowcolor[HTML]{E9E1DE} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Information\\ extraction\end{tabular}}}           & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}Exact maching\\ F1-Score\end{tabular}}                                  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/rajpurkar/squad_v2/viewer/squad_v2/validation?p=52}{SQuAD} \cite{rajpurkar2018know} \vspace{2pt}}                                                                                                                                          \\
\rowcolor[HTML]{D7CCC7} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Relation\\ extraction\end{tabular}}}              & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/YufeiHFUT/BioRED_all_info}{BioRED} \cite{luo2022biored}}                                                                                                                                                                                   \\ \hline
\end{tabular}%
}
\end{table*}

==> latex/tables/tasks_table_3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{rcl}
\multicolumn{3}{c}{{\color[HTML]{000000} \Large \textsc{Healthcare}\vspace{4pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
{\color[HTML]{000000} \textbf{\large \textsc{Tasks}}}                                                                       & {\color[HTML]{000000} \textbf{\large \textsc{Metrics}}}                                                                                  & {\color[HTML]{000000} \textbf{\large \textsc{Datasets}}}                                                                                                                                                                                                                                                                 \\ \hline
\vspace{2pt}
\rowcolor[HTML]{EFEFD2} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Multiple choice\\ questions\end{tabular}}}   & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· MedMCQA \cite{pmlr-v174-pal22a}\\ · PubMedQA \cite{jin2019pubmedqa}\\ · MedQA \cite{jin2020disease}\\ · MMLU \cite{hendrycks2020measuring}\\ · CareQA\end{tabular}}                                                                                   \\
\rowcolor[HTML]{E3EFD6} 
        
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Open-ended\\ medical questions\end{tabular}}}     & {\color[HTML]{656565} \normalsize \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT, ROUGE,\\ BERTScore, MoverScore, \\ Prometheus, Perplexity \end{tabular}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://huggingface.co/datasets/bigbio/meddialog}{MedDialog} \cite{zeng2020meddialog} \\ · \href{https://huggingface.co/datasets/bigbio/mediqa_qa}{MEDIQA2019} \cite{MEDIQA2019} \end{tabular}\vspace{2pt}}  


\\
\rowcolor[HTML]{C8E9D9} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Making diagnosis and treatment\\ recommendations\end{tabular}}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT, ROUGE,\\ BERTScore, MoverScore\\ Prometheus, Perplexity\end{tabular}}  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/BI55/MedText}{MedText} \vspace{2pt}}                                                                                                                                                                                                       \\
\rowcolor[HTML]{CDEBEB} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Writing\\ prescriptions\end{tabular}}}            & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/devlocalhost/prescription-full}{Prescription} \vspace{2pt}}                                                                                                                                                                                \\
\rowcolor[HTML]{C7DBE9} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Clinical\\ note-taking\end{tabular}}}             & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT, ROUGE,\\ BERTScore, MoverScore,\\ Prometheus, Perplexity\end{tabular}} & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://huggingface.co/datasets/har1/MTS_Dialogue-Clinical_Note}{MTS-Dialog} \cite{mts-dialog}\\ · ACI-Bench \cite{aci-bench}\end{tabular} \vspace{2pt}}                                                                                                     \\ 

\rowcolor[HTML]{E1DEE9} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ classification\end{tabular}}}      & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://www.kaggle.com/datasets/chaitanyakck/medical-text/data}{Medical Text for classification} \cite{10.1145/3582768.3582795}\\ · \href{https://www.kaggle.com/datasets/tboyle10/medicaltranscriptions}{Medical Transcriptions}\end{tabular}} \\


\hline
\multicolumn{3}{l}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\
\multicolumn{3}{c}{{\color[HTML]{000000} \large \textsc{NLP}\vspace{4pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\rowcolor[HTML]{E5CFDF} 
{\color[HTML]{656565} \textbf{Summarization}}                                                              & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT, ROUGE,\\ BERTScore, MoverScore,\\ Perplexity, F1-RadGraph\end{tabular}} & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/dmacres/mimiciii-hospitalcourse-meta}{MIMIC-III} \cite{johnson2016mimic}\vspace{2pt}}                                                                                                                                                      \\

\rowcolor[HTML]{EFD6DC} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Question\\ entailment\end{tabular}}}              & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT, ROUGE,\\ BERTScore, MoverScore,\\ Prometheus, Perplexity\end{tabular}}  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/lighteval/med_dialog}{Meddialog} \cite{zeng2020meddialog} \vspace{2pt}}                                                                                                                                                                                                                        \\
%\rowcolor[HTML]{EFD6DC} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ translation\end{tabular}}}         & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore\end{tabular}}              & {\color[HTML]{656565} · 
%\href{https://huggingface.co/datasets/ayoubkirouane/med_en2es}{Med\_English2Spanish} \vspace{2pt}}                                                                                                                                                          \\
\vspace{2pt}

%\rowcolor[HTML]{E9E1DE} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ classification\end{tabular}}}      & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://www.kaggle.com/datasets/chaitanyakck/medical-text/data}{Medical Text for classification} \cite{10.1145/3582768.3582795}\\ · \href{https://www.kaggle.com/datasets/tboyle10/medicaltranscriptions}{Medical Transcriptions}\end{tabular}} \\
%\rowcolor[HTML]{D7CCC7} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Information\\ extraction\end{tabular}}}           & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}Exact maching\\ F1-Score\end{tabular}}                                  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/rajpurkar/squad_v2/viewer/squad_v2/validation?p=52}{SQuAD} \cite{rajpurkar2018know} \vspace{2pt}}                                                                                                                                          \\
\rowcolor[HTML]{E9E1DE} 
{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Relation\\ extraction\end{tabular}}}              & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/YufeiHFUT/BioRED_all_info}{BioRED} \cite{luo2022biored}}         \\ \hline
\end{tabular}%
} \caption{This table presents the tasks evaluated in this paper, listed in different rows. The second column details the metrics used for each task, including Bits per Byte, Byte Perplexity, and Word Perplexity for perplexity measurements. The third column outlines the different benchmarks used for each task.
} \label{tab:tasks_bench_metrics}
\end{table*}

==> latex/tables/tasks_table_4.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[t]
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{rl}
\multicolumn{2}{c}{{\color[HTML]{000000} \Large \textsc{Close-ended}\vspace{4pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
{\color[HTML]{000000} \textbf{\Large \textsc{Tasks}}}                                                                                                                                          & {\color[HTML]{000000} \textbf{\Large \textsc{Datasets}}}                                                                                                                                                                                                                                                                 \\ \hline
\vspace{2pt}
\rowcolor[HTML]{EFEFD2} 
{\color[HTML]{656565} \textbf{\large\begin{tabular}[c]{@{}r@{}} Multiple choice\\ questions\end{tabular}}}   &  {\large \color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· MedMCQA \cite{pmlr-v174-pal22a}\\ · PubMedQA \cite{jin2019pubmedqa}\\ · MedQA \cite{jin2020disease}\\ · MMLU \cite{hendrycks2020measuring}\\ · CareQA\end{tabular}}                                                                                   \\


\rowcolor[HTML]{E3EFD6} 
{\color[HTML]{656565} \textbf{\large \begin{tabular}[c]{@{}r@{}}Prescription\\ writing\end{tabular}}}            & {\large\color[HTML]{656565} · \href{https://huggingface.co/datasets/devlocalhost/prescription-full}{Prescription} \vspace{2pt}}                                                                                                                                                                                \\


\rowcolor[HTML]{C8E9D9} 
{\color[HTML]{656565} \textbf{\large\begin{tabular}[c]{@{}r@{}}Medical text\\ classification\end{tabular}}}      & {\large\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://www.kaggle.com/datasets/chaitanyakck/medical-text/data}{Medical Text for classification} \cite{10.1145/3582768.3582795}\\ · \href{https://www.kaggle.com/datasets/tboyle10/medicaltranscriptions}{Medical Transcriptions}\end{tabular}\vspace{2pt}} \\

\rowcolor[HTML]{CDEBEB} 
{\color[HTML]{656565} \textbf{\large\begin{tabular}[c]{@{}l@{}}Relation\\ extraction\end{tabular}}}                     & {\large \color[HTML]{656565} · \href{https://huggingface.co/datasets/YufeiHFUT/BioRED_all_info}{BioRED} \cite{luo2022biored}}         \\


\hline
\multicolumn{2}{l}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\
\multicolumn{2}{c}{{\color[HTML]{000000} \Large \textsc{Open-ended}\vspace{4pt}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline

\rowcolor[HTML]{C7DBE9} 
        
{\color[HTML]{656565} \textbf{\large\begin{tabular}[c]{@{}r@{}}Open-ended\\ medical questions\end{tabular}}}     &  {\large \color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://huggingface.co/datasets/bigbio/meddialog}{MedDialog} \cite{zeng2020meddialog} \\ · \href{https://huggingface.co/datasets/bigbio/mediqa_qa}{MEDIQA2019} \cite{MEDIQA2019} \end{tabular}\vspace{2pt}}  


\\
\rowcolor[HTML]{E1DEE9} 
{\color[HTML]{656565} \textbf{\large\begin{tabular}[c]{@{}r@{}}Making diagnosis \\ and treatment \\ recommendations \\ \end{tabular}}}   & {\large \color[HTML]{656565} · \href{https://huggingface.co/datasets/BI55/MedText}{MedText} \vspace{2pt}}                                                                                                                                                                                                       \\


\rowcolor[HTML]{E5CFDF} 
{\color[HTML]{656565} \textbf{\large\begin{tabular}[c]{@{}r@{}}Clinical\\ note-taking\end{tabular}}}              & {\large\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://huggingface.co/datasets/har1/MTS_Dialogue-Clinical_Note}{MTS-Dialog} \cite{mts-dialog}\\ · ACI-Bench \cite{aci-bench}\end{tabular} \vspace{2pt}}                                                                                                     \\

\rowcolor[HTML]{EFD6DC} 
{\large \color[HTML]{656565} \textbf{Summarization}}          & {\large\color[HTML]{656565} · \href{https://huggingface.co/datasets/dmacres/mimiciii-hospitalcourse-meta}{MIMIC-III} \cite{johnson2016mimic}\vspace{2pt}}                                                                                                                                                      \\

\rowcolor[HTML]{E9E1DE} 
{\color[HTML]{656565} \textbf{\large\begin{tabular}[c]{@{}r@{}}Question\\ entailment\end{tabular}}}        & {\large\color[HTML]{656565} · \href{https://huggingface.co/datasets/lighteval/med_dialog}{Meddialog} \cite{zeng2020meddialog} \vspace{2pt}}                                                                                                                                                                                                                        \\



 


%\rowcolor[HTML]{EFD6DC} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ translation\end{tabular}}}         & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}BLEU, BLEURT\\ ROUGE, BERTScore\\ MoverScore\end{tabular}}              & {\color[HTML]{656565} · 
%\href{https://huggingface.co/datasets/ayoubkirouane/med_en2es}{Med\_English2Spanish} \vspace{2pt}}                                                                                                                                                          \\


%\rowcolor[HTML]{E9E1DE} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Medical text\\ classification\end{tabular}}}      & {\color[HTML]{656565} Accuracy}                                                                                          & {\color[HTML]{656565} \begin{tabular}[c]{@{}l@{}}· \href{https://www.kaggle.com/datasets/chaitanyakck/medical-text/data}{Medical Text for classification} \cite{10.1145/3582768.3582795}\\ · \href{https://www.kaggle.com/datasets/tboyle10/medicaltranscriptions}{Medical Transcriptions}\end{tabular}} \\
%\rowcolor[HTML]{D7CCC7} 
%{\color[HTML]{656565} \textbf{\begin{tabular}[c]{@{}r@{}}Information\\ extraction\end{tabular}}}           & {\color[HTML]{656565} \begin{tabular}[c]{@{}c@{}}Exact maching\\ F1-Score\end{tabular}}                                  & {\color[HTML]{656565} · \href{https://huggingface.co/datasets/rajpurkar/squad_v2/viewer/squad_v2/validation?p=52}{SQuAD} \cite{rajpurkar2018know} \vspace{2pt}}                                                                                                                                          \\
 \hline
\end{tabular}%
} \caption{This table presents the tasks evaluated in this paper, listed in different rows. The second column details the metrics used for each task, including Bits per Byte, Byte Perplexity, and Word Perplexity for perplexity measurements. The third column outlines the different benchmarks used for each task.
} \label{tab:tasks_bench_metrics}
\end{table}
